Contrastive Learning of Global-Local Video Representations

Contrastive learning has delivered impressive results for various tasks in the self-supervised regime. However, existing approaches optimize for learning representations specific to downstream scenarios, i.e., \textit{global} representations suitable for tasks such as classification or \textit{local} representations for tasks such as detection and localization. While they produce satisfactory results in the intended downstream scenarios, they often fail to generalize to tasks that they were not originally designed for. In this work, we propose to learn video representations that generalize to both the tasks which require global semantic information (e.g., classification) and the tasks that require local fine-grained spatio-temporal information (e.g., localization). We achieve this by optimizing two contrastive objectives that together encourage our model to learn global-local visual information given audio signals. We show that the two objectives mutually improve the generalizability of the learned global-local representations, significantly outperforming their disjointly learned counterparts. We demonstrate our approach on various tasks including action/sound classification, lip reading, deepfake detection, event and sound localization (https://github.com/yunyikristy/global\_local).

==> backup.tex <==

\iffalse
\begin{table}[tp]
\small
\centering
\begin{tabular}{l|ll|cc}
\toprule
Method & Backbone & Pretrained on & LRS$\downarrow$ & LRW$\uparrow$  \\ \hline
WAS~\cite{LRS} & Conv. & N/A & 70.4 & 76.2  \\
STF~\cite{STF:Zhang_2019_ICCV} & ResNet18 & N/A & 51.7 & 83.7 \\
TM-CTC~\cite{TM-seq2seq} & ResNet18 & N/A & 65.0 & - \\
TM-sep2seq~\cite{TM-seq2seq} & ResNet18 & N/A & \underline{49.8} & - \\
LRW~\cite{LRW} & VGG-M & N/A & - & 61.1 \\
Perfect Match~\cite{chung2019perfect} & TC-5 & N/A & - & 71.6 \\
ResNet-LSTM~\cite{stafylakis2017combining} & ResNet34 & N/A & - & 83.0 \\
TwoStream~\cite{TwoStream-lipreading} & I3D & N/A & - & 84.1 \\
DFTN~\cite{DFTN} & ResNet18 & N/A & - & \underline{84.1} \\ \hline
MoCo~\cite{moco:He:2020} & ResNet18 & K-AV-15K & 71.5 & 61.2 \\
CPC~\cite{CPC:oord2018representation} & ResNet18 & K-AV-15K & 66.7 &65.3\\
DPC~\cite{CPC:oord2018representation} & ResNet18 & K-AV-15K & 65.1 & 67.5\\
AVSlowFast~\cite{xiao2020slowfast} & ResNet18 & K-AV-15K & 56.1 & \textcolor{blue}{75.8} \\ 
InfoMax~\cite{videoInfomax} & ResNet18 & K-AV-15K & \textcolor{blue}{53.2}  & 70.7\\\hline
\multirow{3}{*}{Ours} 
  & ResNet18 & K-AV-15K & \textcolor{blue}{47.8} & \textcolor{blue}{83.7} \\
  & ResNet50 & K-AV-15K & 45.0 & 85.5 \\
  & ResNet18 & K-AV-240K & \textbf{45.1} & \textbf{89.2} \\ \bottomrule
\end{tabular}
\caption{Comparison with SOTA on lipreading: LRS (WER, lower is better) and LRW (top-1 accuracy). \underline{Underline} are the best results from the supervised approaches. \textcolor{blue}{Blue text} highlights the comparison of ours with the self-supervised approaches under the same setting.}
% DFTN~\cite{DFTN} ($^{\dagger}$) uses RGB + optical flow; all the other methods use RGB only.
\label{tab:lip-reading-sota}
\end{table}
\fi

\iffalse
\begin{table}[tp]
\centering
\small
\begin{tabular}{l|cl|cc}
\toprule
Method & Backbone & Pretrained on & DFDC (AUC)$\uparrow$  \\ \hline
Capsule~\cite{nguyen2019capsule} & VGG-19 & N/A& 53.3  \\
Multi-task~\cite{Multitask:nguyen2019multi} & Y-shape & N/A & 53.6  \\
HeadPose~\cite{HeadPose:yang2019exposing} & -  & N/A  & 55.9  \\
Two-stream~\cite{TwoStream:zhou2017two} & Inception3 & N/A & 61.4  \\
VA-MLP~\cite{VA-MLP} & - & N/A & 61.9  \\
VA-LogReg~\cite{VA-MLP} & - & N/A & 66.2  \\
Xception-c40~\cite{rossler2019faceforensics++} & XCeption & N/A & 69.7  \\
Xception-c23~\cite{rossler2019faceforensics++} & XCeption & N/A & 72.2  \\
FWA~\cite{FWA:li2018exposing} & - & N/A & 72.7  \\
Meso4~\cite{afchar2018mesonet} & Inception4 & N/A & 75.3  \\
DSP-FWA~\cite{FWA:li2018exposing} & - & N/A & 75.5  \\
Siamese~\cite{emotion-dfdc} & - & N/A & 84.4$^{\dagger}$  \\
MDS~\cite{MDS:chugh2020not} & ResNet18 & N/A & \underline{91.5}$^{\dagger}$  \\ \hline 
MoCo~\cite{moco:He:2020} & ResNet18 & K-AV-15K & 60.2 \\
CPC~\cite{CPC:oord2018representation} &ResNet18 & K-AV-15K & 67.9 \\
DPC~\cite{han:2019:DPC} & ResNet18 & K-AV-15K & 71.2 \\
AVSlowFast~\cite{xiao2020slowfast} & ResNet18 & K-AV-15K & 80.9 \\ 
InfoMax~\cite{videoInfomax} & ResNet18 & K-AV-15K & \textcolor{blue}{85.3}\\\hline
%& Unimodal (DFDC) & ResNet18 & K-AV-15K & 95.5       \\
%& Multimodal (DFDC) & $\checkmark$ & $\checkmark$ & ResNet18 & K-AV-15K & 95.6    \\
\multirow{3}{*}{Ours} & ResNet18 & K-AV-15K  & \textcolor{blue}{90.1} \\
& ResNet50 & K-AV-15K  & 92.7 \\
& ResNet18 & K-AV-240K & \textbf{96.7} \\ \bottomrule
% Ours Atten. (no face cropping)                                   &   $\checkmark$   & $\checkmark$   & 95.0       \\
% Ours Multimodal                                &   $\checkmark$   & $\checkmark$   & 95.6     \\ \bottomrule 
\end{tabular}
\caption{Comparison with SOTA on deepfake detection. For training on DFDC, we use the same training and test splits as \cite{MDS:chugh2020not}. \cite{emotion-dfdc} use the same number of randomly sampled training data (180K). All the numbers of the other SOTA approaches are collected from \cite{MDS:chugh2020not}. All the self-supervised approaches are pretrained on K-AV-15K, and finetuned and tested on the same training and test sets of DFDC. Siamese~\cite{emotion-dfdc} and MDS~\cite{MDS:chugh2020not} ($^{\dagger}$) use audio-visual signals; all other the methods use visual signals only.}
\label{tab:dfdc-sota}
\end{table}
\fi


\begin{table}[t!]
    \centering
    \small
    \begin{tabular}{ccc|lllll}
    \toprule
    V. Enc. & Obj. & Feat. & LRS2$\downarrow$ & LRW$\uparrow$ & DFDC$\uparrow$ & UCF101$\uparrow$ & HMDB51$\uparrow$  \\ \hline
    Both & LG ($\mathcal{L}_{g}$) & LG ($z_v^g$) & 70.9 & 65.3 & 67.9 & 82.3 & 57.1 \\
    Both & Both & LG ($z_v^g$) & 47.6 \textcolor{blue}{($\downarrow$ 23.3)} & 86.8 \textcolor{blue}{($\uparrow$ 21.5)} & 92.6 \textcolor{blue}{($\uparrow$ 24.7)} & 89.2 \textcolor{blue}{($\uparrow$ 6.9)} & 59.9 \textcolor{blue}{($\uparrow$ 2.8)} \\ \hline
    Both & GL ($\mathcal{L}_{l}$)    & GL ($z_v^l$) & 68.6 & 65.1 & 70.3 & 82.1 & 55.6\\
    Both & Both & GL ($z_v^l$) & 46.5 \textcolor{orange}{($\downarrow$ 22.1)} & 88.9 \textcolor{orange}{($\uparrow$ 23.8)} & 95.9 \textcolor{orange}{($\uparrow$ 25.6)} & 88.5 \textcolor{orange}{($\uparrow$ 6.4)} & 58.3 \textcolor{orange}{($\uparrow$ 2.7)} \\ \hline
    GL    & Both & Both & 50.8 & 81.2 & 89.7 & 83.6 & 57.3 \\ 
    Both & Both & Both & \textbf{45.1 \textcolor{green!55!blue}{($\downarrow$ 5.7)}} & \textbf{89.2 \textcolor{green!55!blue}{($\uparrow$ 8.0)}} & \textbf{96.7 \textcolor{green!55!blue}{($\uparrow$ 7.0)}} & \textbf{90.1 \textcolor{green!55!blue}{($\uparrow$ 6.5)}} & \textbf{61.3 \textcolor{green!55!blue}{($\uparrow$ 4.0)}} \\
    \bottomrule
    \end{tabular}
    \vspace{1em}
    \caption{The roles of global and local information on different benchmarks. \textbf{LG} means spatially-local/temporally-global and \textbf{GL} means spatially-global/temporally-local. \textbf{V. Enc.}: visual encoder setup, \textbf{Obj.}: contrastive objective used during pretraining, \textbf{Feat.}: features used in downstream tasks.}
    \label{tab:global-vs-local}
\end{table}

